Just Propagate: Unifying Matrix Factorization, Network Embedding, and LightGCN for Link Prediction

Link prediction is a fundamental task in graph analysis. Despite the success of various graph-based machine learning models for link prediction, there lacks a general understanding of different models. In this paper, we propose a unified framework for link prediction that covers matrix factorization and representative network embedding and graph neural network methods. Our preliminary methodological and empirical analyses further reveal several key design factors based on our unified framework. We believe our results could deepen our understanding and inspire novel designs for link prediction methods.

==> relatedwork.tex <==
\section{Related Work}\label{sec:relatedworks}
This section will briefly review several kinds of collaborative filtering(CF) methods. Then we discuss differences with other most relevant works, especially on interpreting and unifying CF models for the recommendation.

CF is the fundamental recommendation task and plays an essential role in research and industry. CF methods use implicit interactions only and learn low-dimensional vectors to reconstruct historical interactions without using any other side information. Matrix factorization (MF)~\citep{mf1,mf2} models are earlier CF models, which simply project ID features as embeddings and use the inner product as a matching function. Further, in order to capture nonlinear relationships between user-item interactions, models such as NeuMF~\citep{neumf}and LRML~\citep{LRML} use neural networks instead of inner product are proposed. Recently, graph representation learning (GRL) techniques, including network embedding methods (NE) and graph neural networks(GNNs), have shown successes in various graph analysis tasks. Since the recommendation task can be thought of as the link prediction task in the user-item bipartite graph, GRL techniques, i.e., graph-based CF, are naturally introduced.

Although graph-based CF methods, especially LightGCN, have achieved state-of-the-art performance, there lacks a unified framework to help us better understand these CF models in a global view. GF-CF\citep{GF-CF}, the only one, as far as we know, only focuses on the process of the forward process and drives a unified framework only based on low-pass filtering. While in this work, we consider the whole procedure of representation learning, including both the forward and backward process, and result in a more comprehensive framework.
